Trust Stack for Mental Health AI: A Survey of Calibration across Human, Interaction, and AI Layers

Language-based AI is increasingly deployed for mental health support, yet trust is evaluated in interdisciplinary but operationally misaligned ways: NLP and AI work measures robustness, safety, privacy, and explanations, while psychotherapy, HCI, and regulatory work emphasize therapeutic fidelity, lived experience, empathy, and reliance. Empathetic chatbots can elicit strong user trust without commensurate safety, while safer systems are under-trusted when their boundaries are opaque, a calibration gap no single community owns. Through a structured scoping synthesis of 61 papers, we survey this landscape into a three-layer framework separating (L1) human-oriented trust, (L2) interaction-oriented trustworthiness, and (L3) AI-oriented trustworthiness, and map five stakeholder perspectives onto these layers. We outline a research agenda for building socio-technically aligned trustworthy AI for mental health support, highlighting that the central objective should shift from maximizing perceived trust to calibrating human trust to demonstrated interaction- and AI-level trustworthiness.

==> Tables/mindmap.tex <==
% We position human trust factors in mental health as the anchor that defines what “trustworthy” should mean, and map them to interaction and AI mechanisms that operationalize these factors, forming a bidirectional loop for design and evaluation.


Root: 
Trustworthy AI for Mental Health

Layer 1: Layer of Trustworthiness
Human-Oriented Trustworthiness
Interaction-Oriented Trustworthiness
AI-Oriented Trustworthiness

Layer 2: Trustiness dimensions 
Human-Oriented Trustworthiness:
- Trust calibration/acceptance
- Accountability & recourse (user-facing)
- Autonomy & control (user agency)
- Privacy expectations & comfort (perceived)
- Clinical validity & efficacy
- Crisis-handling / escalation

Interaction-Oriented Trustworthiness:
- Usability
- Communication quality 
- Transparency (disclosure)
- Empathy
- Anthropomorphism / agency cues


AI-Oriented Trustworthiness:
- Reliability
- Robustness
- Fairness
- Security
- Safety
- Explainability
- Uncertainty calibration (know-when-not-to-answer)
- Technical privacy (e.g., leakage resistance)

